DABT: A Dependency-aware Bug Triaging Method

In software engineering practice, fixing a bug promptly reduces the associated costs. On the other hand, the manual bug fixing process can be time-consuming, cumbersome, and error-prone. In this work, we introduce a bug triaging method, called Dependency-aware Bug Triaging (DABT), which leverages natural language processing and integer programming to assign bugs to appropriate developers. Unlike previous works that mainly focus on one aspect of the bug reports, DABT considers the textual information, cost associated with each bug, and dependency among them. Therefore, this comprehensive formulation covers the most important aspect of the previous works while considering the blocking effect of the bugs. We report the performance of the algorithm on three open-source software systems, i.e., EclipseJDT, LibreOffice, and Mozilla. Our result shows that DABT is able to reduce the number of overdue bugs up to 12\%. It also decreases the average fixing time of the bugs by half. Moreover, it reduces the complexity of the bug dependency graph by prioritizing blocking bugs.

==> Archive/Archived_text.tex <==
\begin{comment}
\newpage
\appendix

\subsection{Data Preparation}
\begin{itemize}
    \item non-fixed bugs and bugs with no explicit assignment information are considered as invalid bugs, and we only use valid bugs with assignment information in our experiments.
    \item To filter out inactive developers, using the interquartile range (IQR) of bug fix numbers of each developer;  i.e., 
    \begin{equation*}
        \text{IQR} = \text{the third quartile} - \text{the first quartile}
    \end{equation*}
    Higher distributions than IQR are considered as active. We thus consider developers whose bug fix number is higher than IQR as active developers.
\end{itemize}

\subsection{Performance Metrics}
\begin{enumerate}
    \item the \# of correct assignment
    \item the \# of solved bugs
    \item graph complexity
    \item Bug rank
    \item fair distribution among developers
    \item infeasible solving bugs w.r.t. BDG
\end{enumerate}



\subsection{IP model considerations}

\begin{itemize}
    \item This model can be solved using Gurobi implementation in Python.
    \item Based on the experience of a developer, it is expected to have different fixing time for each. Therefore, the bug fixing time should be exclusive for the assignee. Also, not all the bugs have the same amount of time to be solved. The characteristics of a bug are a proper indicator of its fixing time. Therefore, we will predict the time to be solved $c_i^d$ for the bug $i$ and a developer $d$ using the pipeline in Figure~\ref{fig:fixing_time}.
    
    \begin{figure}[!htb]
    \centering
        \includegraphics[width=0.7\textwidth]{figs/fixing_time_prediction.pdf}
        \caption{Fixing time estimation}
        \label{fig:fixing_time}
    \end{figure}
    
    Textual information of a bug, including summary and description, will be converted to a numeric data using word2vec, then we utilize TF-IDF of the its vocabularies as the weight and combine all word2vec information using weighted average. We merge that vector with meta data of the bug, e.g., the component of a bug, the number of comments, the number of votes, the number of CC'ed developers, and the number of bugs it blocks, the number of blocking bugs, assignee, priority, and severity. Finally, Gradient boosting regressor is applied on the output to predict the fixing time. Given a new bug, we can estimate its fixing time per assignee using pre-trained model. \citet{park2011costriage} explored something.
    
    \item Lagrangian decomposition or other model relaxation algorithms can be used to improve the solvability of the IP model, i.e. faster solution times, and the ability to solve larger models.
    
    \item Some papers regarding constraint programming that also have many applications in Artificial Intelligence can be regarded as a way to improve the solving performance of the model.
    \item To make the model more realistic, the objective function (\ref{eq:IP-objective}) can be revised and include other reward or cost coefficient. To address the subjectivity in severity assignment, we will build an LSTM network to give a coefficient per developer for each bug. This coefficient can be generated based on the experience of the developer in the specific component in which the bug is reported and the textual description of a bug, thus ensuring to assign the proper developer to each bug. In the updated formula $s_i$ changes to $c_i^d$, indicating the suitability coefficient of developer $d$ for bug $i$. 
\end{itemize}


\subsection{Results}

\begin{table}[!ht]
\caption{Comparison of different algorithms\label{tab:comp_algorithms}}%
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|rrrr}
        \toprule
        \multicolumn{1}{r}{} & \multicolumn{1}{r}{\textbf{Actual}} & \multicolumn{1}{r}{\textbf{CBR}} & \multicolumn{1}{r}{\textbf{CosTriage}} & \multicolumn{1}{r}{\textbf{RABT}} \\
        \midrule
        \textbf{\# of assigned bugs} &  1,112 & 1,112 & 1,112 & 870 \\
        \textbf{\# of un-assigned bugs} & 0 & 0 & 0 & 242 \\
        \textbf{\# of assigned developers} & 9 & 10 & 10 & 10 \\
        \textbf{Fair distribution among developers ($\sigma$)} & 97.80 & 86.70 & 102.62 & 68.99 \\
        \textbf{\# of overdue bugs} & 914 & 982 & 872 & 234 \\
        \textbf{\# of un-fixed bugs} & 672 & 542 & 601 & 10 \\
        \textbf{Developer/day needed *} & ?? &  &  &  \\
        \textbf{Avg. Fixing days per bug} & 3886.88!! & ! & ! & 25.85 \\
        \textbf{Accuracy of assignments} & - & 41\% & 38\% & 11\% \\
        \textbf{Graph complexity * } &  &  &  &  \\
        \textbf{infeasible solving bugs w.r.t. BDG * } &  &  &  & \\
        \bottomrule
    \end{tabular}
}
\end{table}


\textcolor{red}{Adding Kashiwa paper's result}



\end{comment}

\begin{comment}

\section{Questions}

\begin{itemize}
    \item I really need help regarding the IP model: why its accuracy is super low?
    \item When should I do assignment? How many bugs should be assigned? How it works with SVM per se?
    \item assigning and simultaneously keeping track of the resolved time is super complex! No idea on how to make it simpler. (reopening issue as well)
\end{itemize}

\section{Things done this week}
\begin{itemize}
    \item 
\end{itemize}

\section{Things to be done}
\begin{itemize}
    \item Applying collaborative filtering
    \item Applying CC engagement instead of collaborative filtering as a modification of their problem.
\end{itemize}


\section{Design of experiment}

\subsection{Database}
\subsubsection{Bug details}
\begin{itemize}
    \item id
    \item severity
    \item priority
    \item comment\_count
    \item network (whether solved or in BDG)
    \item open: tracking introducing time
    \item close: when it is solved
    \item blocks: list of the bugs it blocks
    \item depends\_on: list of the bugs blocking it
    \item depth: its depth in BDG
    \item degree: its degree in BDG
    \item status: default is "NEW"
    \item last\_status: it is read from the db
    \item unresolved\_time: The day it is closed - the day it is assigned + 1
    \item cluster: to which subgraph in BDG it belongs
    \item updated: Whether we need to update it
    \item sequence: the sequence of events that the bug goes through
    \item description: bug description
    \item summary: bug summary
    \item assigned\_to
    \item assigned\_to\_id
    \item valid4assignment (whether it is assigned to an active developer in its history)
    \item assigned\_to\_rec: keeping the record of assignments
    \item assigned\_time: keeping track of assignment time
    \item assignment\_accuracy: whether the model assigned it correctly.
    \item component: which components it belongs to
    \item time\_to\_solve: The day it is closed - the day it is assigned + 1
    \item LDA\_category: based on LDA
    
    
    We only add the bug to the network if its last status is not ``depulicate"
    
\end{itemize}

\subsubsection{Developers details}
\begin{itemize}
    \item  email
    \item n: developer's number (starts from 0)
    \item id\_: developer id
    \item name
    \item bugs that are assigned        \item working\_time: how long it took to solve each bug
    \item components: list of components the developer had previous experience in
    \item time\_limit: the default is 30 and if we assign a bug, it will be reduced
    \item LDA\_experience: Its LDA experience
\end{itemize}

\subsubsection{BDG details}
\begin{itemize}
    \item network
    \item undirected\_network
    \item bugs\_dictionary
    \item degree
    \item depth
    \item n\_nodes
    \item n\_arcs
    \item n\_clusters
\end{itemize}

\subsubsection{Simulation details}
\begin{itemize}
    \item bug\_info\_db
    \item bug\_evolutionary\_db
    \item birthday: the starting day of simulation, i.e., 2010-01-01
    \item  testing\_time: the starting day of testing phase, i.e., 2018-01-01
    \item BDG
    \item time: current timestamp
    \item filtered\_date: the current day task
    \item day\_counter
    \item date: current day
    \item update: list of the bugs that should be updated
    \item resolved\_bugs: keeping track of resolved bugs
    \item resolution: which resolution (method) to use
    \item all\_opened\_bugs: list of opened bugs
    \item svm\_model: the model saved
    \item Tfidf\_vect: the model saved
    \item available\_developers: list of feasible developers
\end{itemize}
\end{comment}


\begin{comment}
\section{Information about the original study}
This paper reports on the replication of a paper by \citet{kashiwa2020}, established upon the proposed guidelines for experimental replications~\cite{replication}. 

\citet{kashiwa2020} proposed Released-Aware bug triaging method that aims at increasing the number of bugs fixed by the next release. The method considers the time available before the next release and also keeps in check the bug fixing load on developer. It sets a limit to the numbers of bugs that can be assigned to each developer so that more numbers of bugs can be resolved by next release while also considering the ability of the developer. It regards the bug assignment problem as a multiple knapsack problem to find the optimal combination of bugs and developers. This method prevents bug assignments to be skewed for few experienced developers and also increases the total number of bugs fixed by assigning an optimal number of bugs to each developer.\\



\citet{kashiwa2020} addresses bug triage as multiple knapsack problem to optimize task assignments by finding best possible combination of bug (item) and the developer (knapsack) to maximize the bug-fixing efficiency of the project (objective) under the given time limit (constraint). They extract data on fixed bugs from the BTS and use them to train the SVM and LDA Model. Fixer and bug description data is used to train the SVM to compute the preferences of developer for fixing the bug. So when a new bug $B_j$ is reported, it estimates each developer’s $D_i$ probability (preferences $P_{ij}$) for fixing the bug. The time required to fix a bug by the developer is obtained by the LDA model which categorizes the bugs using the bug description from extracted data and then calculates the average time for each developer to fix each category of bugs(cost list). Hence when a new bug $B_j$ is reported, input its description to trained LDA, bug category is inferred from LDA which then gives the average time taken by Developer $D_i$ to fix bugs in that category k as the bug fixing cost $C_{ij}$ of the new bug.  Then available time slot $T_{i}$ for each developer is obtained based on the upper limit L (predetermined) and total cost of bugs already assigned to them. Bug is then assigned to the suitable developer based on the Preferences $P_{ij}$, cost  $C_{ij}$ and the available time slots $T_{i}$.\\
They conducted the experiment on three projects (Mozilla Firefox, the \scshape{Eclipse} platform and GNU compiler collection (GCC)) dataset. Table outlines the dataset used as training and test data for all the projects (table 1). They only considered fixed bugs (bugs whose status was FIXED) and developers who fixed six or more bugs within six months of their first assignment (active developers) for their experiment (table 2). 

\begin{table}[h!]
\centering
\begin{tabular}{ |c|c|c|c| } 

\hline
Project & Dataset & Date & Period \\
\hline
\multirow{2}{8em}{Firefox} & Training data  & Jul. 5, 2010 – Jul. 4, 2011  & 1 year  \\ 
& Testing data  & Jul. 5, 2011 - Sep. 27, 2011 & 12 weeks  \\ 
\hline
\multirow{2}{8em}{Eclipse Platform} & Training data  & Mar. 22, 2010  Mar. 21, 2011 & 1 year  \\ 
& Testing data  & Mar. 22, 2011 – Jun. 22, 2011 & 3 months   \\ 
\hline
\multirow{2}{8em}{GCC} & Training data  & Dec. 25, 2009 – Dec. 24, 2010  & 1 year  \\ 
& Testing data  & Dec. 25, 2010 – Mar. 25, 2011 & 3 months   \\ 
\hline
\end{tabular}
\caption{Datasets}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c| }  
 \hline
 Projects & No. of all developers & No. of active developers \\  
 \hline
 Firefox & 215 & 19 \\ 
 \hline
 Eclipse Platform & 61 & 20 \\
 \hline
 Gcc & 97 & 23\\
 \hline
\end{tabular}
\caption{Active developers in each dataset}
\end{table}

\citet{kashiwa2020} compared the RABT method with the other two existing methods for bug triaging(CBR and CosTriage). CBR \cite{anvik2006should} considers bug triage as a multi-class classification problem. They trained a multi-class classifier using the past history of bug fixes which estimates each developer’s score for the new bug by extracting its feature vector and applying the classifier. For classification they used SVM, Naive Bayes and C4.5. CBR only considers accuracy and suffers from over-specialization, recommending only the types of bugs that each developer has solved before. Thus, concentrating the task to some experienced developers and thus slows down the bug fixing process. While CosTriage \cite{park2011costriage} method tried to not only optimize the accuracy but also the cost. This method models the developer profile that denotes the developer’s estimated cost for fixing a certain bug type. Bug categories are extracted by applying the LDA to bug description. Then as with CBR, it determines the probability that each developer is appropriate for the bug. Thus, by combining the cost with the possibilities estimated as by CBR, developers are ranked and bug is assigned to the first developer. Both these methods (CBR and CosTriage) do not consider the number of bugs that the developer can address in the given time period.  Thus, assigning more bugs than the developer can resolve and irregular distribution of bugs leads to decrease in the number of bugs fixed before next release. RABT method addresses this problem by setting a Limit to the number of tasks assigned to each developer and thus balancing the load among the developers, which increases the numbers of bugs fixed. While evaluating and comparing these three methods, it shows CosTriage mitigate the task concentration compared to CBR, however, RABT outperforms the CosTriage in this case and thus the bug-fixing time of the developer assigned by RABT also significantly reduces. RABT can also assign more appropriate amount of bugs that developer can fix by the next release, thus reducing the overdue bugs compare to CBR and CosTriage by 30-60\%. Compared to these two methods, RABT also outperforms in reducing the bug fixing time of the project by reducing bug fixing time by 25-46\%. Though, it has been found that the bug assignment accuracy of RABT decreases by 20\% compared to CBR, with accuracy of 74\%. While CosTriage was 2\% lower than that of CBR.

RABT outperforms the existing methods in all the aspects except the accuracy of the assignment, decreasing it by 20\%. Kashiwa states two reasons for the lower accuracy. First, there are other developers that fixed the bug in the same component, yet RABT can assign bug to the developer whose preference is not the highest. Secondly, the case when there is only one developer in the component as the size of training data for each developer varies in size. Even when the assignment is not appropriate and developer needs double fixing time, RABT performs better than the other methods in term of the task distribution, number of bugs the developer can fix in the given time period and the bug fixing time.  They mentioned that the order in which the bugs are assigned impacts the number of bugs fixed by the release. Also, the developers with fewer tasks are not necessarily available to handle tasks as they might be engaged in other project activities. Since RABT overlooks this condition, the developer might be burdened with extra load. RABT performs these case studies on Mozilla Firefox, Eclipse Platform and GNU Gcc and confirms , RABT mitigates the task concentration, assigns  more appropriate number of bugs a developer can fix in the given time period and reduces the bug fixing time.
\end{comment}
